Quantile Surfaces -- Generalizing Quantile Regression to Multivariate Targets

In this article, we present a novel approach to multivariate probabilistic forecasting. Our approach is based on an extension of single-output quantile regression (QR) to multivariate-targets, called quantile surfaces (QS). QS uses a simple yet compelling idea of indexing observations of a probabilistic forecast through direction and vector length to estimate a central tendency. We extend the single-output QR technique to multivariate probabilistic targets. QS efficiently models dependencies in multivariate target variables and represents probability distributions through discrete quantile levels. Therefore, we present a novel two-stage process. In the first stage, we perform a deterministic point forecast (i.e., central tendency estimation). Subsequently, we model the prediction uncertainty using QS involving neural networks called quantile surface regression neural networks (QSNN). Additionally, we introduce new methods for efficient and straightforward evaluation of the reliability and sharpness of the issued probabilistic QS predictions. We complement this by the directional extension of the Continuous Ranked Probability Score (CRPS) score. Finally, we evaluate our novel approach on synthetic data and two currently researched real-world challenges in two different domains: First, probabilistic forecasting for renewable energy power generation, second, short-term cyclists trajectory forecasting for autonomously driving vehicles. Especially for the latter, our empirical results show that even a simple one-layer QSNN outperforms traditional parametric multivariate forecasting techniques, thus improving the state-of-the-art performance.

==> sections/acknowledgment.tex <==
\section{\large Acknowledgment}

This work results from the project DeCoInt$^2$, supported by the German Research Foundation (DFG) within the priority program SPP 1835: ``Kooperativ interagierende Automobile", grant numbers SI 674/11-1.

Additionaly, this work was supported within the project Prophesy (0324104A) funded by BMWi (Deusches Bundesministerium für Wirtschaft und Energie / German Federal Ministry for Economic Affairs and Energy).

==> sections/method_basic_movement_forecast.tex <==
\subsection{Detection of Starting Movements}
\label{subsec:3dcnn_starting_movement_classifcation}

The starting movement detection is modeled as a three class problem, i.e.,
\textit{waiting}, \textit{starting} and \textit{moving}. 
The \textit{starting} class is an auxiliary class, which 
allows to integrate early movement indicators, such as head movements, into the training process. Moreover, it simplifies the 
modeling of the transition between the \textit{waiting} and \textit{moving}
class. $P_{waiting}$, $P_{starting}$, and $P_{moving}$ denote the probabilities assigned by the classifiers to the different classes. The labels of the output data were created manually and are defined as follows: A sequence is labeled as \textit{waiting} if neither the wheel of the bicycle is moving, nor the cyclist is performing a movement that leads to a starting motion. Every frame between the first visible movement of the cyclist which leads to a start and the first movement of the wheel of the bicycle is labeled as \textit{starting}. Finally, every frame after the first movement of the bicycle wheel is labeled as \textit{moving}.

\begin{figure}
	\centering
	\includegraphics[width=0.30\textwidth]{images/ex_netout_scene.pdf}
	\vskip 2mm
	\caption{Exemplary classification output of one scene, with the moving probability $P_{moving}$ (red), the labeled \textit{starting} time (blue), and the labeled \textit{moving} time (green).}
	\vskip -5mm
	\label{fig:ex_net_out}
\end{figure}

Fig. \ref{fig:ex_net_out} shows an exemplary output of the classifier, where the red line represents $P_{moving}$, the blue line is the labeled starting frame and the green line is the labeled moving frame. The output of the classifier should be a zero \textit{moving} probability during phase I (see Fig. \ref{fig:ex_net_out}), the probability should increase in phase II, and should reach a probability of one in phase III. However, sometimes there is no phase II, since there is no visible movement of the cyclist until the wheel of bicycle starts moving.



\subsection{Movement Primitive Detection Using a 3D CNN}
\label{subsec:movement_primitive_detection_cnn}

In this section, we present the use of a 3D CNN with the ResNet architecture to classify starting movements of cyclists. The classification is done frame by frame using the last ten images of a stationary camera.

\subsubsection{Convolutional Neural Network}
\label{subsubsec:cnn}

A CNN architecture mainly consists of convolutional layers which perform convolutions to extract local features from the input and generate feature maps $v_{xy}$, pooling layers to reduce the dimensionality of the feature maps, and a fully connected layer (FCN) at the output.

\small
\begin{equation}
v_{xy} = b_{xy}+\sum_{m=-M}^{M}\sum_{n=-N}^{N}I(x-m, y-n)\cdot K(m+M, n+N)
\label{eq:2dconv}
\end{equation}
\normalsize

Eq.~\ref{eq:2dconv} describes a 2D convolution at the image position $(x, y)$ with the input image $I$ and the filter kernel $K$. The size of the filter kernel in $x$- and $y$-direction is described by $(2M+1, 2N+1)$ for kernels of odd size. After a bias $b_{xy}$ is added to the result of the convolution an activation function, in this case a rectified linear unit (ReLU), is applied. The ReLU outputs $0$ for values smaller than 0, or the value itself for values greater than 0 (Eq.~\ref{eq:relu}):
	
\begin{equation}
f(x)=max(x,0)
\label{eq:relu}
\end{equation}
	
\subsubsection{3D Convolutional Neural Network}
\label{subsubsec:3dcnn}

Since starting movements of cyclists cannot be captured by a single image, 
we added the temporal dimension to the input of the CNN by stacking the last 10 images ($I_{t-9}$ to $I_{t}$) and adding a third dimension to the filter kernel. Fig. \ref{fig:3dcnn_input} shows an example of the 3D CNN input $x^{seq}_t$. The functional behavior of the 3D convolution is shown in Eq.~\ref{eq:3dconv}, where $t$ is the temporal dimension of the image sequence and $2T + 1$ describes the size of the filter kernel in the temporal dimension. By applying the 3D kernel to an image sequence, the extracted features contain information about movements at a certain position.

{\small
\begin{multline}
v_{xyt} = b_{xyt}+ \\ \sum_{m=-M}^{M}\sum_{n=-N}^{N}\sum_{j=-T}^{T}I(x-m, y-n, t-j)\cdot K(m+M, n+N, j+T)
\label{eq:3dconv}
\end{multline}}
\normalsize

\begin{figure}
	\centering
	\includegraphics[width=0.49\textwidth]{images/input_sequence.pdf}
	\vskip 2mm
	\caption{Example input sequence of 3D CNN containing the last 
	ten images for time $t$.}
	\label{fig:3dcnn_input}
	\vskip -3mm
\end{figure}



\subsubsection{Residual Architecture}
\label{subsubsec:res}

The ResNet architecture was introduced by He et al. in 2015 \cite{He.2015}. They propose a network architecture which is easier to train and produces a higher accuracy than conventional CNNs. The authors identified a degradation problem, where adding more layers to a deep model leads to a higher training error. The problem was addressed by adding residual building blocks, where the original input $x$ bypasses a series of convolution layers $F(x)$ and is added to the output resulting in $F(x)+x$. Thus, instead of directly modeling a target function they force the network to model the residual function. By stacking residual blocks, they were able to train a network with 152 layers resulting in substantially better classification results compared to shallower networks. A residual block is depicted in Fig. \ref{fig:net_arch_1}, on the right. Each block has an internal bottleneck structure to reduce the amount of computation. The first $1\times 1\times 1$ convolution represents the input in a lower dimension, followed by an $N\times M\times T$ convolution.

Our network architecture is described in Fig. \ref{fig:net_arch_1} and is based on the network from \cite{He.2015}. To reduce the number of input features, after a batch normalization layer, an initial convolution followed by a max pooling layer is applied. Before the feature maps are passed to the residual blocks, a $1\times 1\times 1$ convolution is carried out to generate 32 feature maps. A residual block consists of 3 sequential repetitions of residual layers with bottleneck architecture. After 6 blocks, resulting in 1024 feature maps, an average pooling is applied, where the result is passed to a fully connected layer followed by a softmax layer to generate probabilities. In order to speed up the training process, batch normalization layers were added at the network input and after every residual block.

The output vector $\hat{y}_t^{cnn}$ of the overall network contains the probabilities of 3 classes: $P_{waiting}$, $P_{starting}$, and $P_{moving}$. 
Our network is trained on the input sequences $x^{seq}_t$ of each individual time step and outputs a feature vector $\hat{y}_t^{cnn}$, which contains the class probabilities.

\begin{figure}
	\centering
	\includegraphics[width=0.49\textwidth]{images/3d_resnet.pdf}
	\vskip 2mm
	\caption{Architecture of the residual 3D CNN. A residual block is depicted in the upper right and the reduction layer in the lower right.}
	\label{fig:net_arch_1}
	\vskip -3.5mm
\end{figure}





\subsection{Movement Primitive Detection Using Smart Devices}
\label{subsec:movement_primitive_detection_sd}

\input{sections/smart_device_movement_primitive_detection}

\subsection{Cooperative Movement Primitive Detection}
\label{sec:cooperative_mp_pred}

\input{sections/coop_movement_primitive_detection}



==> sections/results_basic_movement_forecast.tex <==
\subsection{Movement Primitive Detection}
\label{sec:results_basic_moevement}

\begin{figure*} [h]
	\centering
	\vskip -4mm
	\includegraphics[width=1.7\columnwidth]{"images/f1"}
	\vskip -2mm
	\caption{$F_1$-score (blue), precision (red) and mean detection time (green) over the probability thresholds of all cyclists (left) and instructed cyclists (right).}
	\label{fig:res3dcnn}
	%\vspace{12mm}
	\vskip -2mm
\end{figure*}

\subsubsection{3D CNN}
\label{subsubsec:3dcnn_results}
%trim=0 60 0 105
%\centering
%\includegraphics[width=0.5\textwidth]{"images/f1"}
In this section, we describe the evaluation of the 3D CNN. The dataset we used is divided into a training and a validation set, $s_{train}$ and $s_{val}$. $s_{train}$ consists solely of uninstructed cyclists and makes up 60\% of all measurements. $s_{val}$ consists of all instructed cyclists and additional uninstructed cyclists and was split into two sets $s_{val1}$ and $s_{val2}$ to perform a two-fold cross-validation. $s_{val}$ is split in a way that instructed and uninstructed cyclists are evenly distributed. The classification of the 3D CNN is evaluated on $s_{val}$. To compare the classification results of the 3D CNN to the smart device classifier, we additionally illustrate the results of the instructed cyclists.

The overall results of the classifier are shown in Fig.~\ref{fig:res3dcnn}. To generate the plots, the $F_1$-score, the precision, and $\overline{\delta_t}$ of the classifier are determined (as described in Sec.~\ref{sec_method_evaluation}) for different probability thresholds. The results are plotted over the thresholds from zero to one. The plot on the left contains the results of both folds using all sequences, the right plot contains the results of only the instructed cyclists, respectively. 

Our evaluation shows, that the classifier reaches an $F_1$-score of 90\% at \SI{-0.02}{\second} and 98\% at \SI{0.19}{\second}, on average on the \textit{mixed} data. The evaluation on instructed cyclists produces similar results with an $F_1$-score of 90\% at \SI{-0.07}{\second} and 98\% at \SI{0.14}{\second}. We can see an increase in the $F_1$-score and the precision (blue and red curves) with an increasing threshold due to fewer false positives. The mean detection time $\overline{\delta_t}$ (green) increases with the threshold, because $P_{moving}$ usually increases over time until the maximum probability is reached.

Further analyses showed, that the classifier is robust against small movements of the cyclist and even movements in the background of the cyclist, e.g., a pedestrian walking by. Fig.~\ref{fig:grafic_behind} shows a snapshot of a scene. Two pedestrians, one pushing a bicycle, are passing behind the target cyclist. In Fig. \ref{fig:plot_behind}, the corresponding network output is shown. The passing pedestrians cause a slight increase in $P_{starting}$ (green line, peak $1$ and $2$), however, $P_{moving}$ stays unaffected.

\begin{figure}[h]
	\centering
	\includegraphics[width=0.5\textwidth]{images/action_behind.pdf}
	\caption{Example classification of one scene with two pedestrians passing in the background of the cyclist. The probabilities $P_{waiting}$ (blue), $P_{starting}$ (green) and $P_{moving}$ (red) are shown. Label $\textit{1}$ references the pedestrian on the left pushing a bicycle. Label $\textit{2}$, the pedestrian in the background on the right.}
	\label{fig:plot_behind}
	\vskip -4mm
\end{figure}

\begin{figure}[b]
	\centering
	\includegraphics[width=0.45\textwidth]{images/cropped_walking_behind.png}
	\vskip 2mm
	\caption{Two pedestrians passing in the background of the cyclist.}
	\label{fig:grafic_behind}
\end{figure}

Fig. \ref{fig:failure_plot_behind} (left) shows the network output of a scene with a pedestrian passing very close to the cyclist, which leads to a sharp increase in $P_{moving}$ resulting in a false positive detection. We observed that the network strongly reacts to movements in the area of the bicycle wheels. The passing pedestrian is depicted in Fig.~\ref{fig:grafic_behind2}.

\begin{figure}[h]
	\centering
	\includegraphics[width=0.5\textwidth]{images/cmp170.pdf}
	\vskip 2mm
	\caption{Comparison between the classification output of the 3D CNN (left) and the stacking ensemble (right). $P_{moving}$ of the 3D CNN is falsified by a pedestrian walking in the background, this is compensated in the stacking ensemble output.}
	\label{fig:failure_plot_behind}
	\vskip -4mm
\end{figure}

\begin{figure}[b]
	\centering
	\includegraphics[width=0.393\textwidth]{images/cropped_walking_behind2.png}
	\vskip 2mm
	\caption{Pedestrian passing close to the cyclist.}
	\label{fig:grafic_behind2}
\end{figure}

Another problem are changing environmental conditions, i.e., occlusion, lighting, or weather 
conditions indirectly affecting the detectors performance. 
In our evaluation data, stormy weather is an example for this changing 
environmental conditions. Here, the otherwise steady camera images start to shake, which leads to a noisy output (Fig.~\ref{fig:cmp130}, left).

\begin{figure}[h]
	\centering
	\includegraphics[width=0.50\textwidth]{images/cmp130.pdf}
%	\vskip 2mm
	\caption{Comparison between the classification output $P_{moving}$ of the 3D CNN (left) and the stacking ensemble (right). Here, the camera shakes due to heavy winds.}
	\label{fig:cmp130}
\end{figure}

Since the smart device sensors are not affected by passing VRUs or changing environmental conditions such as weather situations, we can use the output of the smart device classifier to resolve these issues.

% Ich hab hier einen Teil rausgenommen, weil ich denke, dass das in die nächste Subsection gehört

%two sets 60\% $d_1$ and 40\% $d_2$, such that all data, introduced as instructed cyclists, are within the $d_2$. $d_1$ is used to train the base part of the 3D-CNN, no validation and testing does take place at this stage. $d_2$ is further split into $d_{21}$ and $d_{22}$, such that all data, introduced as instructed cyclists, is equally distributed. 
%Both $d_{21}$ and $d_22$ contain a subset $d_{21s}$ and $d_{22s}$ of instructed cyclists, representing are all entries with smart device data. The subset is used to evaluate the motion primitive detection and the mixture of experts model. 

%For the two-fold cross validation $d_{21}$/$d_{21s}$ is first used as train and $d_{22}$/$d_{22s}$ as test set, than vise versa. The average result of the cross validation is presented in the following.




\subsubsection{Smart Devices}
\label{subsubsec:result_smart_devices}
In this section, we describe the evaluation of the smart device based starting movement detector. 
For evaluation of the smart device based approach only the set of instructed cyclist can be considered. 

The overall results of the smart device based detector are shown in Fig.~\ref{fig:final_cmp}. 
Our evaluation shows that the classifier reaches an $F_1$-score of 80\% at a mean detection time of \SI{0.16}{\second}. 
We observe that the precision of the classifier is low compared to the 
the camera based 3D CNN approach. 
The classifier produces many false positives and is sensitive to small motions of the cyclist.
Most of them occur due to movements of cyclists while they are waiting, e.g., when the cyclist is preparing the pedal to start, but is not starting yet. Other false positives 
are due to seesawing movement, i.e., swaying from one leg to the other.
This results in an activity pattern similar to the one observed just before starting.
Many of those false positives can be filtered, i.e., by averaging the last prediction. But this comes at the cost of reduced detection speed.
This shows that for the smart device based detector a high threshold has to be chosen in order to achieve a larger $F_1$-score. Eventually an additional smoothing is necessary.
Despite of the high number of false positive detections, the detection can be a valuable source of information for a cooperative classifier, since it is less affected by changing environmental conditions or passing VRUs.
In case of occlusion the smart devices can be the only source of information left. Hence, the camera and smart device based classifier can complement each other. 

\subsection{Cooperative Movement Primitive Detection}
\label{sec:results_cooperative_prediction}
In this section, we describe the evaluation of the cooperative approach.
As before, the evaluation is performed via a two-fold cross-validation on the set of instructed cyclists.
The smart device and cooperative movement detector have to share the same training set. This is compensated by performing a nested five-fold cross-validation over the VRUs in the respective training fold. 
The smart device based model is fitted on the training data of the nested training folds. The predictions of 
the nested validations folds are concatenated creating the training basis for fitting the stacking ensemble model.

The results of the cooperative approach are depicted in Fig.~\ref{fig:final_cmp}.
The classifier reaches an $F_1$-score of 90\% at \SI{-0.09}{\second} and 98\% at \SI{0.13}{\second} 
evaluated on the instructed cyclists. The cooperative stacking ensemble approach outperforms the smart device and 3D CNN based approaches concerning the $F_1$-score. 
The cooperative approach produces an $F_1$-score of $99$\% and a mean detection time of \SI{0.24}{\second} for threshold values greater than $0.98$. 
%Concerning our evaluation data of instructed cyclists this is a single false starting detection. 
The cooperative approach combines robustness while retaining a low mean detection time. 

We observe an increased robustness against false positive detections. 
In Fig.~\ref{fig:failure_plot_behind}, this is illustrated for a scene with a 
passing pedestrian behind a waiting cyclist. While there are \textit{moving} probability peaks in the solely 3D CNN based approach (Fig. \ref{fig:failure_plot_behind}, left), there is no notable peak for the stacking ensemble (Fig.~\ref{fig:failure_plot_behind}, right).

The cooperative approach offers also increased robustness concerning 
environmental conditions, e.g., shaking camera. As depicted in Fig.~\ref{fig:cmp130}, the noise in the \textit{moving} probability predictions is tremendously reduced allowing a clear starting detection. 

\begin{figure}[h]
	\centering
	\includegraphics[width=0.42\textwidth]{images/final_cmp.pdf}
%	\vskip 2mm
	\caption{$F_1$-score (blue) and mean detection times (green) over the probability thresholds of the instructed cyclists for the different models, cooperative stacking ensemble (solid), 3D CNN (dotted) and smart device based (crossed).}
	\label{fig:final_cmp}
%	\vskip -4mm
\end{figure}
